VeritasFi: An Adaptable, Multi-tiered RAG Framework for Multi-modal Financial Question Answering

Retrieval-Augmented Generation (RAG) is becoming increasingly essential for Question Answering (QA) in the financial sector, where accurate and contextually grounded insights from complex public disclosures are crucial. However, existing financial RAG systems face two significant challenges: (1) they struggle to process heterogeneous data formats, such as text, tables, and figures; and (2) they encounter difficulties in balancing general-domain applicability with company-specific adaptation. To overcome these challenges, we present VeritasFi, an innovative hybrid RAG framework that incorporates a multi-modal preprocessing pipeline alongside a cutting-edge two-stage training strategy for its re-ranking component. VeritasFi enhances financial QA through three key innovations: (1) A multi-modal preprocessing pipeline that seamlessly transforms heterogeneous data into a coherent, machine-readable format. (2) A tripartite hybrid retrieval engine that operates in parallel, combining deep multi-path retrieval over a semantically indexed document corpus, real-time data acquisition through tool utilization, and an expert-curated memory bank for high-frequency questions, ensuring comprehensive scope, accuracy, and efficiency. (3) A two-stage training strategy for the document re-ranker, which initially constructs a general, domain-specific model using anonymized data, followed by rapid fine-tuning on company-specific data for targeted applications. By integrating our proposed designs, VeritasFi presents a groundbreaking framework that greatly enhances the adaptability and robustness of financial RAG systems, providing a scalable solution for both general-domain and company-specific QA tasks. Code accompanying this work is available at https://github.com/simplew4y/VeritasFi.git.

==> bak.tex <==
-------- algorithm --------
% \KwIn{
%     $\mathcal{D}_{\text{human}}$: A human-annotated dataset of triplets $(q, p^+, p^-)$, where $q$ is a query, $p^+$ is a relevant chunk (positive), and $p^-$ is an irrelevant chunk (negative); \\
%     $\mathcal{Q}_{\text{target}}$: A set of queries for the target company; \\
%     $\mathcal{C}_{\text{target}}$: The document corpus for the target company; \\
%     $\mathcal{M}_{\text{base}}$: The pre-trained base re-ranker model; \\
%     $\mathcal{R}$: The retrieval module for fetching candidate chunks; \\
%     $\mathcal{L}_{\text{anno}}$: The LLM-based annotator for automated labeling;
% }

% \begin{algorithm}[t]
% \caption{Two-Stage Re-ranker Fine-Tuning}
% \label{alg:reranker_training}
% \KwIn{
%     Human-annotated general dataset $\mathcal{D}_{\text{human}} = \{(q, p^+, p^-), \dots\}$; \\
%     Target company queries $\mathcal{Q}_{\text{target}}$ and corpus $\mathcal{C}_{\text{target}}$; \\
%     Base re-ranker model $\mathcal{M}_{\text{base}}$, Retriever $\mathcal{R}$, LLM-Annotator $\mathcal{L}_{\text{anno}}$
% }
% \KwOut{Specialized re-ranker model $\mathcal{M}_{\text{specialized}}$}
% \BlankLine

% \SetKwFunction{FMain}{TrainContrastive}
% \SetKwProg{Fn}{Function}{:}{}
% \Fn{\FMain{$\mathcal{M}$, $\mathcal{D}_{\text{train}}$}}{
%     \ForEach{training step}{
%         Sample a query $q$ from $\mathcal{D}_{\text{train}}$\;
%         Let $\mathcal{P}_q, \mathcal{N}_q$ be the positive and negative sets for $q$\;
%         Sample one positive chunk $p^+ \in \mathcal{P}_q$\;
%         Sample $K$ negative chunks $\mathcal{N}^- \subset \mathcal{N}_q$\;
%         Compute logits $\mathbf{s} = [\text{Score}(q, p^+), \dots, \text{Score}(q, p^-_K)]$ with model $\mathcal{M}$\;
%         Compute loss $\mathcal{L} = -\log\left(\frac{e^{s^+}}{e^{s^+} + \sum_{j=1}^{K} e^{s^-_j}}\right)$\;
%         Update $\mathcal{M}$ by minimizing $\mathcal{L}$\;
%     }
%     \Return{$\mathcal{M}$}
% }

% \BlankLine
% \tcc{--- Stage 1: Training the General Financial Re-ranker ---}
% $\mathcal{D}_{\text{aug}} \gets \emptyset$\;
% \ForEach{$(q, p^+, p^-) \in \mathcal{D}_{\text{human}}$}{
%     $q_{\text{aug}}, p^+_{\text{aug}}, p^-_{\text{aug}} \gets \text{ApplyEntityAbstraction}(q, p^+, p^-)$\;
%     Add $(q_{\text{aug}}, p^+_{\text{aug}}, p^-_{\text{aug}})$ to $\mathcal{D}_{\text{aug}}$\;
% }
% $\mathcal{M}_{\text{general}} \gets$ \FMain{$\mathcal{M}_{\text{base}}$, $\mathcal{D}_{\text{aug}}$}\;

% \BlankLine
% \tcc{--- Stage 2: Rapid Onboarding for Target Company ---}
% $\mathcal{D}_{\text{auto}} \gets \emptyset$\;
% \ForEach{$q \in \mathcal{Q}_{\text{target}}$}{
%     $\mathcal{C}_q \gets \mathcal{R}(q, \mathcal{C}_{\text{target}})$ \tcp*{Retrieve candidate chunks}
%     $\mathcal{P}_q, \mathcal{N}_q \gets \mathcal{L}_{\text{anno}}(q, \mathcal{C}_q)$ \tcp*{Label with LLM-Annotator}
%     Add $(q, \mathcal{P}_q, \mathcal{N}_q)$ to $\mathcal{D}_{\text{auto}}$\;
% }
% $\mathcal{M}_{\text{specialized}} \gets$ \FMain{$\mathcal{M}_{\text{general}}$, $\mathcal{D}_{\text{auto}}$}\;

% \BlankLine
% \Return{$\mathcal{M}_{\text{specialized}}$}
% \end{algorithm}


 % \begin{algorithm}[t] \caption{Re-ranker Fine-Tuning Pipeline} \label{alg:reranker} \KwIn{Query set $\mathcal{Q}$, Document corpus $\mathcal{C}$, Retrieval module $\mathcal{R}$, Base reranker model $\mathcal{M}$} \KwOut{Trained reranker $\mathcal{M}^\ast$} \BlankLine \textbf{Step 1: Automated Data Annotation} \\ \ForEach{$q \in \mathcal{Q}$}{ Retrieve candidate chunks $\mathcal{C}_q \gets \mathcal{R}(q, \mathcal{C})$\; \ForEach{$c \in \mathcal{C}_q$}{ Annotate relevance $y \in \{0,1\}$ using LLM-based annotator with prompt template\; } Construct positive set $\mathcal{P}_q = \{c \mid y=1\}$, negative set $\mathcal{N}_q = \{c \mid y=0\}$\; } \BlankLine \textbf{Step 2: Data Augmentation (Entity Abstraction)} \\ \ForEach{chunk $c \in \mathcal{C}$}{ Generate abstracted versions $\{c^{(1)}, c^{(2)}, c^{(3)}, c^{(4)}\}$ via LLM with masking strategies\; } Build augmented dataset $\mathcal{C}^\prime$ with varying abstraction levels\; \BlankLine \textbf{Step 3: Contrastive Learning Data Construction} \\ \ForEach{$q \in \mathcal{Q}$}{ \ForEach{training step}{ Sample $p^+ \sim \mathcal{P}_q$ (positive)\; Sample $K$ negatives $\mathcal{N}^- \subset \mathcal{N}_q \cup$ random($\mathcal{C}$)\; Compute logits $\mathbf{s} = [s^+, s^-_1, \ldots, s^-_K]$ with model $\mathcal{M}$\; Update $\mathcal{M}$ by minimizing: \[ \mathcal{L} = -\log\frac{e^{s^+}}{e^{s^+} + \sum_{j=1}^K e^{s^-_j}} \] } } \BlankLine \textbf{Step 4: Two-Stage Training} \\ \begin{enumerate}[leftmargin=*] \item \textit{Stage 1 (Generalization):} Train $\mathcal{M}$ on augmented dataset $\mathcal{C}^\prime$ to acquire domain-general ability\; \item \textit{Stage 2 (Specialization):} Fine-tune $\mathcal{M}$ on raw annotated data $\{\mathcal{P}_q, \mathcal{N}_q\}$ to adapt to target company\; \end{enumerate} \BlankLine \Return{$\mathcal{M}^\ast$} \end{algorithm}

 
% \begin{algorithm}[t]
% \caption{Re-ranker Fine-Tuning}
% \label{alg:reranker}
% \KwIn{Query set $\mathcal{Q}$, Document corpus $\mathcal{C}$, Retrieval module $\mathcal{R}$, Base reranker model $\mathcal{M}$}
% \KwOut{Trained reranker $\mathcal{M}^\ast$}

% \tcp{Step 1: Automated Data Annotation}
% \ForEach{$q \in \mathcal{Q}$}{
%     Retrieve candidate chunks $\mathcal{C}_q \gets \mathcal{R}(q, \mathcal{C})$\;
%     \ForEach{$c \in \mathcal{C}_q$}{
%         Annotate relevance $y \in \{0,1\}$ using LLM-based annotator\;
%     }
%     Build $\mathcal{P}_q = \{c \mid y=1\}$ and $\mathcal{N}_q = \{c \mid y=0\}$\;
% }

% \tcp{Step 2: Data Augmentation (Entity Abstraction)}
% \ForEach{chunk $c \in \mathcal{C}$}{
%     Generate abstracted versions $\{c^{(1)}, c^{(2)}, c^{(3)}, c^{(4)}\}$ via LLM\;
% }
% Obtain augmented dataset $\mathcal{C}^\prime$\;

% \tcp{Step 3: Contrastive Learning}
% \ForEach{$q \in \mathcal{Q}$}{
%     \ForEach{training step}{
%         Sample $p^+ \sim \mathcal{P}_q$, negatives $\mathcal{N}^- \subset \mathcal{N}_q \cup$ random($\mathcal{C}$)\;
%         Compute logits $\mathbf{s} = [s^+, s^-_1, \ldots, s^-_K]$\;
%         Update $\mathcal{M}$ by minimizing $\mathcal{L} = -\log \frac{e^{s^+}}{e^{s^+} + \sum_{j=1}^K e^{s^-_j}}$\;
%     }
% }

% \tcp{Step 4: Two-Stage Training}
% Train $\mathcal{M}$ on $\mathcal{C}^\prime$ (generalization)\;
% Fine-tune $\mathcal{M}$ on $\{\mathcal{P}_q,\mathcal{N}_q\}$ (specialization)\;

% \Return{$\mathcal{M}^\ast$}
% \end{algorithm}
 
% \begin{algorithm}[t]
% \caption{Re-ranker Fine-Tuning Pipeline}
% \label{alg:reranker}
% \KwIn{Query set $\mathcal{Q}$, Document corpus $\mathcal{C}$, Retrieval module $\mathcal{R}$, Base reranker model $\mathcal{M}$}
% \KwOut{Trained reranker $\mathcal{M}^\ast$}

% \tcp{Step 1: Automated Data Annotation}
% \ForEach{$q \in \mathcal{Q}$}{
%     Retrieve candidate chunks $\mathcal{C}_q \gets \mathcal{R}(q, \mathcal{C})$\;
%     \ForEach{$c \in \mathcal{C}_q$}{
%         Use LLM annotator with structured prompt and few-shot rules\;
%         Assign binary relevance label $y \in \{0,1\}$ with reasoning trace\;
%     }
%     Build positive set $\mathcal{P}_q = \{c \mid y=1\}$ including direct matches, contextual support, and fuzzy time matches\;
%     Build negative set $\mathcal{N}_q = \{c \mid y=0\}$\;
% }

% \tcp{Step 2: Data Augmentation (Entity Abstraction)}
% \ForEach{chunk $c \in \mathcal{C}$}{
%     Generate four abstracted variants using LLM-guided masking strategies:\;
%     (1) Replace target company with ``the company''\;
%     (2) Mask product models and personal names with placeholders (e.g., Product A, Person B)\;
%     (3) Replace target company with a competitor name from pool (Tesla, NIO, XPeng, BYD)\;
%     (4) Apply full abstraction: replace all entities with placeholders (Company A, Product B, Person C)\;
% }
% Construct augmented dataset $\mathcal{C}^\prime$ with multiple abstraction levels\;

% \tcp{Step 3: Contrastive Learning}
% \ForEach{$q \in \mathcal{Q}$}{
%     \ForEach{training step}{
%         Sample one positive $p^+ \sim \mathcal{P}_q$\;
%         Sample $K$ negatives $\mathcal{N}^- \subseteq \mathcal{N}_q \cup$ random($\mathcal{C}$)\;
%         Compute logits $\mathbf{s} = [s^+, s^-_1, \ldots, s^-_K]$ using reranker $\mathcal{M}$\;
%         Update $\mathcal{M}$ by minimizing loss: 
%         $\mathcal{L} = -\log \frac{e^{s^+}}{e^{s^+} + \sum_{j=1}^K e^{s^-_j}}$\;
%     }
% }

% \tcp{Step 4: Two-Stage Training}
% Stage 1 (Generalization): Train $\mathcal{M}$ on abstracted dataset $\mathcal{C}^\prime$ to learn domain-general semantics\;
% Stage 2 (Specialization): Fine-tune $\mathcal{M}$ on raw annotated pairs $\{\mathcal{P}_q, \mathcal{N}_q\}$ for company-specific adaptation\;

% \Return{$\mathcal{M}^\ast$}
% \end{algorithm}



-------- sections --------
% \begin{enumerate}[leftmargin=*]
% \item \textbf{Data Augmentation}
% % XBH 2025/9/18
% To improve model generalization and reduce overfitting to specific entity names, we construct multiple abstracted versions of the company dataset. This process is designed to disentangle the model's learned semantic reasoning from its reliance on memorized, explicit entity-specific facts.
% % disentangles the influence of explicit entity knowledge from general semantic reasoning.
% The abstraction process is implemented through a unified Python framework that interacts with a large language model, guided by the carefully designed prompts.
% % This setup allows us to flexibly adjust the granularity of entity masking and to ensure consistent placeholder assignment within each instance, while maintaining fidelity to the factual structure of the original text.
% % Queries, positive and negative samples are all processed, and the pipeline incorporates multi-threaded execution, error recovery with exponential backoff, and logging to guarantee robust large-scale processing.
% Within this framework, we design three abstraction strategies that progressively mask entity-specific information:
% \textbf{i)} Replaces mentions of the target company (e.g., Zeekr, Lotus Technology) with neutral placeholders, while other company names with randomly sampled competitor name from a predefined pool (e.g., Tesla, NIO, XPeng, BYD). % simulating cross-company generalization scenarios, while with neutral placeholders, while  % such as “the company,” while retaining other company names.
% % The second preserves company names but replaces specific product models and individual names, including executives, board members, and shareholders, with abstract placeholders such as Product A or Person B. 
% \textbf{ii)} Replaces specific product models and individual names, including executives, board members, and shareholders, with abstract placeholders.
% \textbf{iii)} Applies full entity abstraction, where all mentions of companies, products, and individuals are consistently replaced with abstract placeholders. %such as Company A, Product B, and Person C.
% By generating parallel corpora under these three strategies, we obtain multiple versions of the same dataset that reflect different levels of entity masking, which allows  us to train re-ranker under altered conditions. The comparative results across different abstraction levels provide the basis for choosing the most robust and generalizable strategy.

% \item \textbf{Automated Data Annotation}
% % WHW
% Manual annotation of retrieval outputs presents significant practical challenges that motivated our development of an automated solution. First, human annotation is time-intensive, particularly given the large volume of document chunks generated by our Multi-path Retrieval pipeline. More critically, any modifications to system components, whether in the Financial Filings Pre-processing pipeline or retrieval strategies, require complete re-annotation of the dataset, creating substantial maintenance overhead. Additionally, when annotation tasks are distributed among multiple annotators, subjective differences in relevance judgment inevitably introduce inconsistencies in labeling quality, potentially compromising the effectiveness of subsequent re-ranker training. These factors collectively required the implementation of an automated annotation process that ensures both scalability and consistency.

% To optimize the re-ranker's performance, we implement an automatic annotation module that generates high-quality training data from the retrieval stage outputs. This module employs a specialized LLM-based annotator to label document chunks as relevant or irrelevant for given queries, creating the positive and negative samples essential for re-ranker fine-tuning through contrastive learning. The annotation process operates on the comprehensive set of retrieved chunks from our Multi-path Retrieval pipeline, ensuring that the training data reflects the actual distribution of candidate documents the re-ranker encounters during inference.

% The annotation process centers on a carefully engineered prompt design that combines explicit relevance criteria with few-shot examples to guide the LLM's judgment. The prompt establishes three primary relevance categories: direct answer match (chunks containing specific data or explicit answers), contextual support (chunks providing essential background or calculation basis), and fuzzy time period match (chunks discussing the same topic within different timeframes). To ensure consistent and accurate annotations, the system uses a structured response format that requires binary relevance decisions accompanied by analytical reasoning. This approach enables batch processing of large-scale retrieval output while maintaining annotation quality through clear guidelines and standardized evaluation criteria. The complete annotation prompt template and detailed relevance assessment criteria are provided in Appendix~\ref{app:annotation_prompt}.


% \item \textbf{2-stage training} We first train the re-ranker on the augmented dataset, where all specific company related features are processed with the optimal abstraction strategy. In this stage, the re-ranker is considered to be trained on the generalized data, and expected to acquire the financial-domain-specific ability based on the SEC filing documents; on the second stage, we use the raw data (automatically annotated pos/neg chunks) to simulate the onboarding process of transfer the general re-ranker to a new company, the specific re-ranker would have superior gain in performance but more limited to that specific company.

% \item \textbf{Contrastive Learning}
% To optimize the LLM-based reranker for our specific financial domain, we employ supervised fine-tuning (SFT) using contrastive learning. We utilize the FlagEmbedding framework to fine-tune the \texttt{bge-reranker-v2-gemma} model with carefully constructed positive and negative sample pairs.

% Our training data construction proceeds as follows: for each query $q$, we first collect all chunks retrieved by our retrieval modules and annotate them to identify truly relevant chunks as positive samples $\mathcal{P}_q = \{p^+_1, \ldots, p^+_n\}$ and irrelevant ones as negative samples. To enhance negative sample diversity and difficulty, we build the negative set $\mathcal{N}_q = \{p^-_1,\ldots,p^-_m\}$ in two ways: (1) including retriever-identified chunks that are actually irrelevant, and (2) randomly sampling additional chunks from the entire corpus. This strategy not only ensures sufficient negative samples but also captures "hard negatives"—high-similarity chunks that the retriever mistakenly considers relevant.

% The SFT training data is then structured as:
% \begin{equation}
% \mathcal{D} = \big\{\langle q, \mathcal{P}_q, \mathcal{N}_q, prompt \rangle\big\},
% \end{equation}
% where each training quadruple contains the query, lists of positive and negative chunks, and a standardized prompt template. For each query $q$ in a training step, a mini-batch is constructed containing one positive sample $p^+ \in \mathcal{P}_q$ and $K$ negative samples $\mathcal{N}^- = \{p^-_1, p^-_2, \ldots, p^-_K\} \subset \mathcal{N}_q$. The model computes a set of relevance scores, or logits, $\mathbf{s} = [s^+, s^-_1, \ldots, s^-_K]$, where $s_i = \text{Score}(q, p_i)$.

% To facilitate this contrastive learning objective, the set of $K+1$ candidates is temporarily treated as an \textit{ad-hoc} set of classes for the current query $q$. The task is thus transformed into a classification problem where the model must correctly identify $p^+$ as the single positive class (target index 0) among all candidates $\{p^+, p^-_1, \ldots, p^-_K\}$.
% The training objective is the standard Cross-Entropy Loss applied over the $(K+1)$ scores, targeting the positive sample. The loss function is thus defined as:
% \begin{equation}
% \mathcal{L} = -\log\left(\frac{e^{s^+}}{e^{s^+} + \sum_{j=1}^{K} e^{s^-_j}}\right)
% \end{equation}
% This objective compels the model to maximize the score of the positive sample ($s^+$) relative to all negative samples ($s^-_j$), thus learning the distinctions necessary to differentiate between relevant and irrelevant content.
% \item \textbf{Evaluation} 
% \end{enumerate}


% \subsubsection{Contrastive Learning Objective}
% Both fine-tuning stages are driven by supervised fine-tuning (SFT) on a contrastive learning objective. We utilize the FlagEmbedding framework to fine-tune the \texttt{bge-reranker-v2-gemma} model with carefully constructed positive and negative sample pairs.

% Our training data construction proceeds as follows: for each query $q$, we first collect all chunks retrieved by our retrieval modules and annotate them to identify truly relevant chunks as positive samples $\mathcal{P}_q = \{p^+_1, \ldots, p^+_n\}$ and irrelevant ones as negative samples. To enhance negative sample diversity and difficulty, we build the negative set $\mathcal{N}_q = \{p^-_1,\ldots,p^-_m\}$ in two ways as mentioned in Stage 2 training.
%(1) including retriever-identified chunks that are actually irrelevant, and (2) randomly sampling additional chunks from the entire corpus. This strategy not only ensures sufficient negative samples but also captures "hard negatives"—high-similarity chunks that the retriever mistakenly considers relevant.







-------- table --------
% \begin{table*}[ht]
% \centering
%     \setlength{\tabcolsep}{5pt} % 调整列之间的距离
%     \renewcommand{\arraystretch}{1.3} % 调整行高
% \caption{Ablation study: End to End Performance (top10)}
% \label{tab:ablation}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{l|l|cccc}
% \hline
% \textbf{Dataset} & \textbf{Config} & \textbf{Faithfulness} & \textbf{Response Relevancy} & \textbf{Context Recall} & \textbf{Context Precision} \\ \hline
% \multirow{6}{*}{Zeekr} 
%     & GraphRAG            & -- & -- & -- & -- \\
%     & LightRAG            & -- & -- & -- & -- \\
%     & BM25                & 0.8199 & 0.6296 & 0.3034 & 0.4471 \\
%     & Faiss               & 0.8141 & 0.6961 & 0.3651 & 0.5103 \\
%     & BM25 + Faiss        & 0.8320 & 0.6950 & 0.3603 & 0.5110 \\ 
%     & \ourmodel{}         & 0.6524 & 0.8196 & 0.5778 & 0.3133 \\ \hline
% \multirow{6}{*}{Lotus} 
%     & GraphRAG            & -- & -- & -- & -- \\
%     & LightRAG            & -- & -- & -- & -- \\
%     & BM25                & 0.8769 & 0.7902 & 0.3721 & 0.5403 \\
%     & Faiss               & 0.9305 & 0.8140 & 0.4554 & 0.5044 \\
%     & BM25 + Faiss        & 0.9089 & 0.7790 & 0.4819 & 0.5678 \\ 
%     & \ourmodel{}         & 0.6595& 0.8939 & 0.5762 & 0.3909 \\ \hline
% \multirow{6}{*}{Finder} 
%     & GraphRAG            & -- & -- & -- & -- \\
%     & LightRAG            & -- & -- & -- & -- \\
%     & BM25                & 0.7859 & 0.5314 & 0.2073 & 0.3013 \\
%     & Faiss               & 0.8282 & 0.5772 & 0.2154 & 0.3857 \\
%     & BM25 + Faiss        & 0.8472 & 0.6010 & 0.1854 & 0.3918 \\ 
%     & \ourmodel{}         & 0.6010 & 0.6048 & 0.2392 & 0.3080 \\ \hline
% \multirow{6}{*}{FinanceBench} 
%     & GraphRAG            & -- & -- & -- & -- \\
%     & LightRAG            & -- & -- & -- & -- \\
%     & BM25                & 0.6648 & 0.3256 & 0.2939 & 0.1532 \\
%     & Faiss               & 0.8213 & 0.6319 & 0.5083 & 0.3592 \\
%     & BM25 + Faiss        & 0.7551 & 0.5275 & 0.4600 & 0.2810 \\ 
%     & \ourmodel{}         & 0.6904 & 0.7514 & 0.4917 & 0.3720 \\ \hline
% \multirow{6}{*}{FinQA Bench} 
%     & GraphRAG            & -- & -- & -- & -- \\
%     & LightRAG            & -- & -- & -- & -- \\
%     & BM25                & 0.7253 & 0.7260 & 0.7325 & 0.2784 \\
%     & Faiss               & 0.7830 & 0.7677 & 0.7588 & 0.2910 \\
%     & BM25 + Faiss        & 0.8070 & 0.7476 & 0.7473 & 0.3958 \\ 
%     & \ourmodel{}         & 0.7708 & 0.8029 & 0.7330 & 0.3344 \\ \hline
% \end{tabular}%
% }
% \end{table*}
